Reward Learning using Structural Motifs in Inverse Reinforcement Learning

The Inverse Reinforcement Learning (\textit{IRL}) problem has seen rapid evolution in the past few years, with important applications in domains like robotics, cognition, and health. In this work, we explore the inefficacy of current IRL methods in learning an agent's reward function from expert trajectories depicting long-horizon, complex sequential tasks. We hypothesize that imbuing IRL models with structural motifs capturing underlying tasks can enable and enhance their performance. Subsequently, we propose a novel IRL method, SMIRL, that first learns the (approximate) structure of a task as a finite-state-automaton (FSA), then uses the structural motif to solve the IRL problem. We test our model on both discrete grid world and high-dimensional continuous domain environments. We empirically show that our proposed approach successfully learns all four complex tasks, where two foundational IRL baselines fail. Our model also outperforms the baselines in sample efficiency on a simpler toy task. We further show promising test results in a modified continuous domain on tasks with compositional reward functions.

==> sections/11_contributions.tex <==
\section{Contributions}\label{sec:contributions}


==> sections/51-faq.tex <==
\newpage
\section{Frequently Asked Questions}\label{app:faq}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Novelty}
\paragraph{Q1: How does your work differentiate with Icarte et al.~\cite{lrm2020}?}

The work that is closest to ours is by Icarte et al.~\cite{lrm2020} -- where the authors learn RMs for partially observable RL tasks from trajectories. However, efficacy of the approach is shown in 2D discrete domains, with the authors noting the challenge of showcasing them in 3D continuous domain due to the intractability of state space explosion. While [1] motivates our choice to use RM as the chosen structural motif architecture (as opposed to other available FSA ontologies), but to the best our knowledge, learning the motif on continuous 3D domains with complex logic (see SMIRL Algorithm) is not undertaken in prior works. While this difference can be argued as meagre for 2D toy like domains, but is significant for continuous domains, because `Tabu search' for state space is computationally infeasible in such complex domains. Thus, this insight is more applicable in solving IRL in real-world robotic or embodied-ai domains commensurate with the motivation of our work.

\paragraph{Q2: Does `LRM+MaxEntIRL' imply that you've plugged one existing solution into another?}

No, it surprisingly does not! The motivation of our work is to show that current baseline IRL approaches (including, but not limited to MaxEntIRL) is unable to learn the reward function only from expert demonstrations when there is an underlying (non-Markovian) latent structure driving the trajectories. We show that imbuing the same baselines with the latent structure enables most common IRL methods to circumvent this limitation. The supplementary materials contain our experiments with SMIRL working with other IRL approaches like approaches based on state-marginal matching w/ forward KL divergence (not just MaxEntIRL). 

Based on this motivation (and to establish our hypothesis), it was not only intended, but \textbf{required} to use MaxEntIRL (as a commonplace IRL baseline) and show the efficacy of our approach.

\paragraph{Q2.2: Did we use LRM~\cite{lrm2020} to learn the RMs?} No that would be a misconception.
% - it is not accurate. 
It is worth noting that learning FSA or Reward Machine (RM) from trajectories have already been introduced earlier. However, in all related papers, including~\cite{lrm2020}, this is limited to 2D-discrete domains (where Tabu Search of sub-states is plausible), with the authors noting the challenge of showcasing them in 3D continuous domain due to the intractability of state space explosion. While~\cite{lrm2020} motivates our choice to use RM as the chosen structural motif architecture (as opposed to other available FSA ontologies), but to the best our knowledge, learning the motif on continuous 3D domains with complex logic (see SMIRL Algo) is not undertaken in prior works.

\paragraph{Q3: Is the assumption of a `\textbf{Perfect Labelling Function}' realistic?}
The labelling function in the continuous (Reacher) domain simply assigns truth values to the robot arm fingertip's position being within the circumference of the colored balls (the ball's radius being the implicit error margin from its center if needed for pedagogy). Considering the pixel labelling accuracy of commonplace, off-the-shelf pre-trained image semantic segmentation models available, the assumption of such a labelling function is realistic and reasonable.

\paragraph{Q4: It is not clear if the labelling function would encode prior knowledge about the reward function by itself, which should not be allowed in IRL.}
Here, we define the `labelling function' as an abstract term that captures any function that assigns a truth value of the environment at the current time step, $t$ -- thus, it \textbf{does not} encode any prior knowledge about the reward function itself (see Appendix~\ref{app:supp-materials} Definition 1.1). 

To exemplify, a concrete realization of such a 'labelling function' could be an image semantic segmentation model (e.g. Mask-RCNN) that labels a fluent \texttt{is\_coffee-cup} to true, however, without encoding any prior knowledge of whether the agent held the coffee cup apriori to the current time step. Furthermore, we have updated our definition of the labelling function in Appendix A 1.1 to include a time parameter for better clarity, i.e., $\mathcal{F}_L$ -> $\mathcal{F}_L(t)$.


\paragraph{Q5: Would there be IRL problems to make it infeasible to apply SMIRL?}
Yes certainly. Any multi-objective cases could be deemed as a cursory example. Essentially, cases where the latent reward model cannot be represented by a FSA, then SMIRL would not apply, as presented.

% \paragraph{Q3: What practical problem domains do you think this approach can be applied to?}

% \paragraph{Computational Efficiency}: See appendix C.1 
% \RS{Implementation Details}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{ROUGH WORK -DELETE}

% In order to compensate for performance variability across different underlying RL algorithm implementations~\cite{shengyi2022the37implementation}, we repeat the experiments using OpenAI Stable-Baseline3 (SB3) and spinup frameworks respectively.

% \begin{figure}[h]
% \begin{minipage}[c]{0.68\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{imgs/IRL/reward_function_t3.pdf}
% \end{minipage}
% % \,
% \begin{minipage}[c]{0.3\textwidth}
% \centering
% \caption{\textbf{Qualitative Evaluation in Office World}. The \textbf{learned} FSA structural motif (RM) and weights for Office Gridworld \textit{Task 3: Fetch \& Deliver `Coffee' and `Mail'}. We can see some artifacts of the SMIRL algorithm~\ref{alg:LRM-MaxEntIRL} here with nodes $u_2$ and $u_4$. The first transition from $u_0$ to $u_1$ comes from the fact that the expert trajectories go through \texttt{D} while going to \texttt{c}.}
%     \label{fig:reward_function_t3}
% \end{minipage}
% \end{figure}

% \section{Rough Notes (To be Removed)}\label{appendix:notes}
% \subsection{GAIL~\cite{ho2016generative} review}
% Also see Finn et al.'s~\cite{finn2016guided} concurrent work on using adversarial learning for IRL.

% \subsection{VDB~\cite{peng2018variational} Review}
% \bibliography{main, bibs/irl}



==> sections/90_broader_impact.tex <==
% =====================================================================
% =====================================================================
% \newpage
%  See \href{https://medium.com/@NeurIPSConf/getting-started-with-neurips-2020-e350f9b39c28}{Guidelines}: Authors are asked to include a section in their submissions discussing the broader impact of their work, including possible societal consequences — -both positive and negative.
% =====================================================================
\section*{Broader Impact}\label{impact}
% =====================================================================
 

==> sections/99_acknowledgements.tex <==
% % \newpage
% % =====================================================================
% \section*{Acknowledgements}
% % =====================================================================
 
